On the Impact of the Communication Model on Realisability

Multiparty Session Types (MPST) provide a type-theoretic foundation for specifying and verifying communication protocols in distributed systems. MPST rely on the notion of global type which specifies the global behaviour and local types, which are the projections of the global behaviour onto each local participant. A central notion in MPST is realisability - whether local implementations derived from a global specification correctly realise the intended protocol under a given communication model. While realisability has been extensively studied under peer-to-peer semantics, it remains poorly understood in alternative communication models such as bag-based, causally ordered, or synchronous communications. In this paper, we develop a unified framework for reasoning about realisability and subtyping across a spectrum of communication models. We show that the communication model does not impact the notion of subtyping, but that it impacts the notion of realisability. We introduce several decision procedures for subtyping checking and realisability checking with complexities ranging from NLOGSPACE to EXPSPACE depending on the assumptions made on the global types, in particular depending on their complementability and the size of a given complement.

==> content/discussion-deadlock-free-realizability-and-safe-realizability.tex <==
\etienne{TODO: retrouver les éléments de la discussion dans les versions antérieures ou dans la réponse au reviewer}

==> content/intro.tex <==
% !TEX root =  ../main.tex
%!TEX spellcheck = en_GB

The design and verification of communication protocols in concurrent and distributed systems is a central concern in programming languages. A prominent formalism is Multiparty Session Types (MPST)—a type-theoretic framework that enables specification and static verification of structured interactions among multiple communicating entities~\cite{DBLP:conf/concur/VasconcelosH93,HondaYC08,10.1145/2873052,DBLP:conf/icdcit/YoshidaG20}. MPST  define a global communication protocol that can be projected into local types for each participant, ensuring communication safety and deadlock-freedom.

In this work, we focus on the \emph{realisability problem}, a foundational question in the theory of session types,  that concerns the soundness of the projection mechanism:
the realisability problem asks whether the local types obtained by projecting a global communication specification can be safely used for restricting processes interactions to the original global protocol.

This problem is central to the goal of \emph{correct-by-construction} protocol design, as it ensures that local implementations derived from a specification do not introduce communication mismatches, deadlocks, or unintended behaviours. In the literature on MPST, this challenge has appeared under various names, including \emph{implementability} and \emph{projectability}, reflecting different points of view on the same core issue, with some subtle differences in their definitions. In this work, we adopt the term \emph{realisability}, following the terminology and the spirit of the definition introduced by Alur~\emph{et al}~\cite{DBLP:journals/tcs/AlurEY05} almost a decade before the introduction of multiparty session types. 

The goal of this paper is to tackle the realisability problem for multiparty session types in the context of \emph{arbitrary} communication models. Most existing works on MPST assume a peer-to-peer communication model, where each pair of participants communicates through a dedicated FIFO channel. However, real-world systems often employ diverse communication paradigms, such as unordered message delivery (bag-based), mailbox-based communication, or bus-based systems. Each of these models introduces unique challenges and behaviours that can significantly impact the realisability of global types.

Some prior works have explored realisability under specific communication models,
most of the times either the synchronous model, or the asynchronous peer-to-peer FIFO model. Our framework, on the opposite, is parametric in the \emph{communication model}, allowing us to reason uniformly across all communication models that fit in our framework.
This includes bags, bus, peer-to-peer, mailbox, causally ordered, synchronous, with or without bounded buffering, and combinations of these.

Another distinctive feature of our approach is that we aim at a decision procedure
for realisability rather than a characterisation of realisable global types.
In particular, we do not seek syntactic conditions on global types that guarantee realisability, neither do we consider a priori syntactic restrictions like sender-driven
choices in the definition of global types. Moreover, not only the semantics of
global types, and the notion of realisabitity, but also the decision procedure itself
that we propose are all parametric in the communication model.

Aside from a decision procedure for realisability, we also introduce and study some related notions on global types:

\begin{description}
    \item[complementability] we study whether a global type admits another global type 
    that captures exactly the set of all the behaviours that the first one rejects.
    This notion is closely related to realisability, as we show that realisability implies complementability, and, in turn, that complementability is a key ingredient in our decision procedure for realisability;

    \item[semantic subtyping\footnote{This notion should not be confused with the subtyping notion for \emph{local} types~\cite{Dezani_Ciancaglini_2016}, and by \emph{semantic subtyping} we refer to the notion defined by Castagna and Frisch~\cite{DBLP:conf/icalp/CastagnaF05}.}] we study whether all behaviours accepted by a global type $\gt$ also are allowed by another global type $\gt'$; we observe that this 
    
    \item[communication model monotonicity] we study how realisability is affected when the communication model changes; in particular, we investigate whether a global type $\gt$ that is realisable in a communication model $\acommunicationmodel$

\end{description}
    
\todo[inline]{reprendre autour d'ici}    
    
    can be safely replaced by another global type $\gt'$ that allows more behaviours than $\gt$, while preserving realisability.
    are not allowed by the original global type;
    the ability to construct a global type that captures all behaviours that are complementary (i.e., not allowed) with respect to a given global specification,
the notion of \emph{subtyping} for global types in our setting. Subtyping is a crucial concept in MPST, as it allows for protocol refinement and extension while preserving safety properties. We provide a semantic definition of subtyping that is independent of the communication model, demonstrating that subtyping relations remain consistent across different communication paradigms.

Our main contribution is the identification of a family of communication models, that we call causally-closed for which we can reduce realisability to realisability in the synchronous model, provided that the behaviours of the projection are quasi-synchronous, orphan and deadlock free. Intuitively, a communication model $\acommunicationmodel$ is causally-closed if for each execution in $\acommunicationmodel$ all causally equivalent (up-to permutations of causally independent actions) executions are also contained in $\acommunicationmodel$. Moreover, an execution is quasi-synchronous if it is causally equivalent to an execution where all sent messages can be immediately received.
Now, it is known that realisability in the synchronous model is generally undecidable. 
A key insight of our work is the connection between \emph{realisability} and a property we call \emph{complementability}: the ability to construct a global type that captures all behaviours that are complementary (i.e., not allowed) with respect to a given global specification. 
It turns out that if the complement of a global type is given (or can be computed) then realisability in the synchronous model is decidable.

In the rest of the introduction we give three examples to motivate our choices and results.
\todo[inline]{parler plus de model de communication}

\subsection{ Global Types as Automata for Real-World Protocols}
As mentioned above, we adopt the view of \emph{global types as automata} where transitions capture exchanges between participants. This automaton-based perspective supports precise reasoning about the evolution of protocol states, accommodating branching, concurrency, and synchronisation.
It is more general than the standard "process-algebra" approach as it admits: 1) mixed choice 2) non sender-driven choice 3) some form of parallel behaviour. 

Take for instance a simplified variant of the MQTT publish/subscribe protocol. Two clients, $c_1$ and $c_2$, communicate through a multi-threaded broker. 
Each client may independently send a publish ($p$) message to their corresponding broker thread ($b$ or $b'$), which forwards to the other client which itself responds with an acknowledgment ($a$). 
When a client has finished to publish it send an end message to the broker. 
When all clients have finished, the broker sends a final acknowledgement and the protocol terminates. 
This global behaviour is depicted in Figure \ref{fig:mqtt-globaltype}. 
For readability reasons, we borrow for this example a BPMN inspired notation where nodes labelled with $\|$ to represent thread creation and thread joins, whereas $+$ nodes represent choices or merge of distinct branches. A similar notation has been used in~\cite{DBLP:conf/popl/LangeTY15}. We can "compile" this formalism to finite state automata (when the Petri net underlying the BPMN-like process is 1-safe, or more generally bounded). We illustrate the compilation to a finite state automaton on Figure~\ref{fig:mqtt-subtype}.

\begin{figure}
    \include{figures/mqtt-globaltype.tex}
    \caption{The MQTT global type}\label{fig:mqtt-globaltype}
\end{figure}

\begin{figure}
    \include{figures/mqtt-subtype.tex}
    \caption{A subtype of the MQTT global type and its representation as an automaton.}\label{fig:mqtt-subtype}
\end{figure}



Crucially, the choice of who sends first is not centralised—either client may initiate communication at any time, and the protocol loops accordingly. More precisely, the global type is not sender-driven, as for instance the initial state of the automaton in Figure~\ref{fig:mqtt-subtype} offers a choice between $\gtlabel{c_1}{b}{p}$ and $\gtlabel{c_2}{b'}{p}$. 
This is a common pattern in real-world protocols, where multiple participants can initiate communication independently\footnote{Another example, that we will not detail here, could come from the WebSocket protocol used by
Internet clients for low-latency, full-duplex communication with a server.
After the initial HTTP \emph{Upgrade} handshake, the channel becomes a persistent bidirectional byte stream.  
Either endpoint, the client or the server, may send a frame at any moment. 
The concurrency is even stronger than in MQTT: messages cross in flight, and neither side knows who
will speak next.}.
Despite not being \emph{sender-driven}, this global type is \emph{realisable} in our setting. 

\subsection{Beyond P2P Semantics: the Need for General Communication Models}
Historically,  research on asynchronous MPST has predominantly focused on peer-to-peer communications. However, in practice, many systems are built on top of different communication models, such as unordered (or bag-based), mailbox-based, causally ordered, or bus-based communications. Moreover, as mentioned above the question of implementability has been generally confined to adding some constraints on the syntax of global types (e.g., sender-driven choice that admits only non-mixed choice where sends are performed from the same participant). Such constraints respond to general properties that may seem arbitrary and loosely connected to the two guarantees mentioned above: session conformance and deadlock freedom. 

In this paper, we have a two-fold objective; we aim at:
\begin{enumerate}
\item introducing a theory that is parametric on the communication model,
\item weakening the constraints on global types that guarantee implementability.  
\end{enumerate}

The communication models mentioned before form a hierarchy (see Figure \ref{fig:communication-models-hierarchy}) from more relaxed to more constrained communication models, either in terms
of executions~\cite{DBLP:conf/fm/ChevrouH0Q19}, or in terms of message sequence 
charts~\cite{DBLP:journals/pacmpl/GiustoFLL23}.
Several interesting properties turn out to be monotonic in the communication model in the following sense: if a property is satisfied in a communication model, then it is preserved for more relaxed (resp. more constrained) ones. 
This  is true, for instance, when checking for reachability of a configuration,
for unspecified receptions (the first message in a queue cannot be received by its
destination process), orphan messages (i.e., messages sent by a peer but never received), etc.
Unfortunately, deadlock-freedom, and therefore deadlock-free realisability, are not monotonic.
To better understand this, take the following  two examples. First, consider an example of a global type (in standard MPST syntax) that is realisable in the peer-to-peer model but not in the mailbox one:  $$\gt_1 = \gtlabel{p}{q}{\msg_1} ;\  \gtlabel{r}{q}{\msg_2} ;\  \mathsf{end}.$$
 This global type is realisable in the peer-to-peer model, 
because the projection $p\parallel q \parallel r= !\msg_1 \parallel ?\msg_1.?\msg_2\parallel !\msg_2$ is deadlock-free and session conformant. However, this global type is not realisable in the mailbox model, where all incoming messages of process $q$ are stored in a unique FIFO queue,
because $\msg_2$ could be sent and hence stored in the queue before $\msg_1$  and cause a deadlock.
Second, consider this example where the converse happens: 
%%
$$ 
\begin{array}{lll}
\gt_2 & = & \gtlabel{p}{q}{\msg_1} ;\  \textcolor{red}{\gtlabel{p}{r}{\msg_2}} ;\  \gtlabel{p}{q}{\msg_3} 
        ;\  \textcolor{blue}{\gtlabel{q}{r}{\msg_4}} ;\ \mathsf{end} 
\\
& + & \gtlabel{p}{q}{\msg_1'} ;\  \textcolor{blue}{\gtlabel{q}{r}{\msg_4}} ;\  \gtlabel{q}{p}{\msg_3'} 
        ;\  \textcolor{red}{\gtlabel{p}{r}{\msg_2}} ;\ \mathsf{end}  
\end{array}
$$
%%
This global type $\gt_2$ is depicted in Figure~\ref{fig:gt2}, it features two possible
scenarios, starting either with $\msg_1$ or $\msg_1'$, (that  are depicted on the left). 
It is not realisable in the peer-to-peer model, because the projection 
$p\parallel q \parallel r$ also admits the interaction where  $p$ and $q$ follow the first scenario, but $r$ follows the second scenario, resulting in a non synchronisable interaction (also depicted in Figure~\ref{fig:gt2}). However, this global type is realisable in the mailbox model, because the messages sent to $r$ are stored in a unique FIFO queue, and their order in the queue, is sufficient for  $r$ to  not confuse the two scenarios.
Moreover, this global type, as well as the previous one, are realisable in the synchronous communication model, where ambiguity is resolved by the message ordering.   
\begin{figure}
    \begin{tikzpicture}[scale=0.7]
        \begin{scope}
            \newproc{0}{p}{-2.7};
            \newproc{2}{q}{-2.7};
            \newproc{4}{r}{-2.7};

            \newmsgm{0}{2}{-0.3}{-0.3}{1}{0.5}{black};
            \newmsgm{0}{4}{-1.0}{-1.0}{2}{0.25}{red};
            \newmsgm{0}{2}{-1.7}{-1.7}{3}{0.5}{black};
            \newmsgm{2}{4}{-2.4}{-2.4}{4}{0.5}{blue};
        \end{scope}

        \begin{scope}[xshift=7cm]
            \newproc{0}{p}{-2.7};
            \newproc{2}{q}{-2.7};
            \newproc{4}{r}{-2.7};

            \newmsgm{0}{2}{-0.3}{-0.3}{1'}{0.5}{black};
            \newmsgm{2}{4}{-1.0}{-1.0}{4}{0.5}{blue};
            \newmsgm{2}{0}{-1.7}{-1.7}{3'}{0.5}{black};
            \newmsgm{0}{4}{-2.4}{-2.4}{2}{0.25}{red};
        \end{scope}

        \begin{scope}[xshift=14cm]
            \newproc{0}{p}{-2.7};
            \newproc{2}{q}{-2.7};
            \newproc{4}{r}{-2.7};

            \newmsgm{0}{2}{-0.3}{-0.3}{1}{0.5}{black};
            \newmsgm{0}{4}{-1.0}{-2.4}{2}{0.25}{red};
            \draw[>=latex,->] (0,-1.45) -- node [below, pos = 0.25] {$\msg_{3}$} (2,-1.45);
            \newmsgm{2}{4}{-1.95}{-1.95}{4}{0.5}{blue};
        \end{scope}

    \end{tikzpicture}
    \caption{The two interactions specified by $\gt_2$, and another unspecified interaction that happens in the projected system in the p2p semantics}\label{fig:gt2}
\end{figure}
%%


These two examples show that realisability is not monotonic,
and suggest that every new communication model should prompt the development of a new ad hoc theory of realisable global types, with its own syntactic conditions. 
% In particular the framework proposed by Stutz et al. \cite{DBLP:conf/ecoop/Stutz23}, which is the closest approach to ours (cfr. the Related Work section) is not amenable to a generalisation to a generic communication model.

%\subsection{Subtyping: Protocol Flexibility and Safe Refinement}
%While exact protocol descriptions are useful for specification, real systems often require adaptability—for example, to accommodate extensions, fallback behaviours, or optional features. This motivates the introduction of \emph{subtyping}: a mechanism for safely refining global types without compromising realisability.
%Returning to the MQTT example, suppose we define a \emph{subtype} of the protocol where only one client is allowed to publish, see Figure~\ref{fig:mqtt-subtype}.
%
%In our setting, we give a semantic definition of subtyping, based on the idea that a global type
%$\gt$ denotes a set of executions $\executionsofcfsms{\gt}{\acommunicationmodel}$ that is parameterised by a communication model $\acommunicationmodel$. We therefore say that $\gt$ is a subtype of $\gt'$ in a communication model $\acommunicationmodel$ if 
%$\executionsofcfsms{\gt}{\acommunicationmodel}\subseteq \executionsofcfsms{\gt'}{\acommunicationmodel}$. 
%However, it turns out that the communication model does not impacts our notion of subtyping essentially because global types also admit
%    a MSC-based semantics that is agnostic of the communication model and that defines the same semantic subtyping relation.


\todo[inline]{subsection{Monotonic behavior}
TODO}

\subsection{Subtyping: Protocol Flexibility and Safe Refinement}
While exact protocol descriptions are useful for specification, real systems often require adaptability—for example, to accommodate extensions, fallback behaviours, or optional features. This motivates the introduction of \emph{subtyping}: a mechanism for safely refining global types without compromising realisability.
Returning to the MQTT example, suppose we define a \emph{subtype} of the protocol where only one client is allowed to publish, see Figure~\ref{fig:mqtt-subtype}.

In our setting, we give a semantic definition of subtyping, based on the idea that a global type
$\gt$ denotes a set of executions $\executionsofcfsms{\gt}{\acommunicationmodel}$ that is parameterised by a communication model $\acommunicationmodel$. We therefore say that $\gt$ is a subtype of $\gt'$ in a communication model $\acommunicationmodel$ if 
$\executionsofcfsms{\gt}{\acommunicationmodel}\subseteq \executionsofcfsms{\gt'}{\acommunicationmodel}$. 
However, it turns out that the communication model does not impacts our notion of subtyping essentially because global types also admit
    a MSC-based semantics that is agnostic of the communication model and that defines the same semantic subtyping relation.



\subsection{Contributions}
Summin up, we make the following contributions.
\begin{itemize}
    \item Global type subtyping is a notion that is independent of the communication model (Theorem~\ref{thm:subtyping-agnostic-communication-model}).
    % \item For a fixed communication model, realisability is monotonic in subtyping (Theorem~\ref{thm:realisability-subtyping})
    \item As mentioned above, deadlock-free realisability is not monotonic in the communication model; however, if a global type is deadlock-free realisable in a communication model that contains all synchronous executions, then this global is also realisable in the synchronous model (Theorem~\ref{thm:pp-realizability-implies-synch-realizability}).
    \item It is decidable to verify whether $\gt$ is a subtype of $\gt'$" when $\gt$ and $\gt'$ are realisable (Corollary~\ref{cor:subtyping-decidability}), and more generally when $\gt'$ is complementable  together with few extra assumptions (Theorems~\ref{thm:subtyping-decidability} and \ref{thm:subtyping-decidability-2}).
    \item We show that realisability implies complementability, and that any existing framework in which MPST are realisable "by construction" hides a complementation procedure (Theorem~\ref{thm:complement}). 
    %We explicit a generic complementation procedure with a doubly exponential blowup in the size of the global type, and we give alternative complementation procedures with linear increase in the size of the global in a few cases, like when the global types involves at most three participants, or when all choices are sender-driven (Theorem~\ref{thm:complementation-procedures}).
    \item We show that it is decidable to veriify if  $\gt$ is realisable in a communication model $\acommunicationmodel$ assuming that a complement of $\gt$ is provided. The problem is decidable in PSPACE for the synchronous communication model, and in EXPSPACE for $\ppmodel$, $\bagmodel$, $\causalmodel$, and more generally for any "causally closed", "regular" communication model (Theorem~\ref{thm:decidability-of-implementability-in-p2p})
\end{itemize}


\todo[inline]{rewrite contribution}

\subsubsection*{Outline.} The paper is organised as follows: Section~\ref{sec:preliminaries} introduces the necessary background on executions, Message Sequence Charts, communication models and communicating finite state machines. 
MPST, realisability and complementability are introduced in Section~\ref{sec:global_types}. Finally Section~\ref{sec:decidability}  shows  our results on the reduction of realisability to the synchronous communication model based on the notion of effectively complementable global types.  
Section \ref{sec:concl} concludes with some final remarks and discusses related works.

This paper extends and revise the work in \cite{DGLP25}
\todo[inline]{add more here}

==> figures/mqtt-bad.tex <==
\begin{tikzpicture}[scale=1.5, every node/.style={transform shape}]
\newproc{0}{c_1}{-2.2};
\newproc{1}{b}{-2.2};
\newproc{2}{c_2}{-2.2};

\newmsge{0}{1}{-0.3}{-0.3}{p}{0.5}{black};
\newmsge{1}{2}{-0.9}{-1.5}{p}{0.15}{black};
\newmsge{2}{1}{-0.9}{-1.5}{end}{0.15}{black};
% \newmsgm{2}{1}{-2}{-2}{4}{0.5}{black};
\end{tikzpicture}


==> proofs/lem-eventual-termination-can-be-checked-on-mscs-for-p2p.tex <==
\begin{proof}
    Let $\cfsms=\projectionof{\gt}$.
    \begin{description}
        \item[$\Rightarrow$]
            Let $e\in\executionsofcfsms{\acceptcompletion{\cfsms}}{\acommunicationmodel}\setminus \executionsofcfsms{\cfsms}{\acommunicationmodel}$.
            By the left-hand equality, $e$ is a strict prefix of some
            $e' \in \executionsofcfsms{\cfsms}{\acommunicationmodel} \subseteq \executionsofcfsms{\acceptcompletion{\cfsms}}{\acommunicationmodel}$;
            hence $\cfsms$ can extend $e$, so the reached configuration is not a dead-lock.
        \item[$\Leftarrow$]
            First inclusion is trivial because every word of $\executionsofcfsms{\cfsms}{\acommunicationmodel}$ is accepted by $\cfsms$.
            For the reverse inclusion, let $e\in\executionsofcfsms{\acceptcompletion{\cfsms}}{\acommunicationmodel}$
            If $e\in \executionsofcfsms{\cfsms}{\acommunicationmodel}$ we are done; otherwise deadlock freedom supplies an extension $e'$ of $e$ that is in
             $\executionsofcfsms{\acceptcompletion{\cfsms}}{\acommunicationmodel}$; iterate until a configuration of $\cfsms$ in which all peers are final is met. 
            The concatenation of the successive extensions belongs to $\executionsofcfsms{\cfsms}{\acommunicationmodel}$ and has $e$ as prefix.
    \end{description}
\end{proof}

==> proofs/lem-pp-is-causally-closed.tex <==
% !TEX root =  ../main.tex
%!TEX spellcheck = en_GB
Observe that not all communication models are causally closed. It is the case for $\ppmodel$,  but it is immediate  to see that the property is not valid  for $\synchmodel$. Take for instance  MSC $M$ in Fig.~\ref{fig:rsc_ex},  its linearisation 
$!m_1!m_2?m_1?m_2!m_3?m_3$ 
  does not belong to $\linearisationsof{M_c}{\synchmodel}$.  The following lemma gives examples of causally-closed communication models, the proof is in Appendix \ref{app:lemmacausallyclosed}.

\begin{restatable}[]{lemma}{lemppiscasuallyclosed}\label{lem:pp-is-causally-closed}
	$\executionsofmodel{\ppmodel}$, $\executionsofmodel{\causalmodel}$, and $\executionsofmodel{\bagmodel}$ are causally-closed.
\end{restatable}


==> proofs/thm-sender-driven-choice-complementation.tex <==
Next we give some intuitions about the complementation procedure described in Def.~\ref{def:complement-of-a-sender-driven-gt}, and then introduce the notion of residuation.

For a sequence of arrows $w\in\Arrows^*$, let
 $\stateof{\gt,s}{w}$ denote the state of $\gt$ reached after reading $w$ starting from
state $s$ (recall that $\gt$ is deterministic); note that $\stateof{\gt,s}{w}$ may be
undefined. 

Intuitively, a state $\comp{s}$ of $\comp{\gt}$ is reached after a word $w$ when $\mscof{w}\not\in\existentialmsclanguageof{\gt}$. The difficult point is that we are not in position to accept any sequence of arrows that start with $w$: it might be the case that $\mscof{w\cdot w'}$ is in $\existentialmsclanguageof{\comp{\gt}}$ for some 
sequence of arrows $w'$; still, if this is the case, the first arrow that involves $p$ in $w'$ would then necessarily be one of the arrows labelling an outgoing transition of $s$ in $\gt$. For this reason, $\comp{\gt}$ conservatively rejects $w\cdot w'$ when this is the case.

%It might be wondered whether this is not too drastic and if this could not cause to incidentally reject an MSC $M$ that is not in $\existentialmsclanguageof{\gt}$. 
The reason why  every $M\not\in\existentialmsclanguageof{\gt}$ belongs to $\existentialmsclanguageof{\comp{\gt}}$, is that 
\emph{at least one} sequence of arrows $w$ such that $\mscof{w}=M$ is in $\languageofnfa{\comp{\gt}}$. More precisely, any sequence of arrows $w$ such that the run of $w$ on $\comp{\gt}$ remains as long as possible in the states of $\gt$ will be accepted.

In order to formalise this intuition, we define the notion of residuation. 

\begin{defi}[Residuation]\label{def:residuation}
    Let $\gt$ be a global type with sender-driven choice. The residuation
    $\residat{s}{\gt}{M}$ of a MSC $M$ from a state $s$ of $\gt$ 
    is the pair $(w,M_r)$ defined by induction on the number of events of $M$ as follows.
    \begin{enumerate}
        \item if there are $p,q,m,s_1,M_1$ such that $M=\mscof{\gtlabel{p}{q}{m}}\cdot M_1$,
        and $(s,\gtlabel{p}{q}{m},s_1)$ is a transition of $\gt$,
        then $\residat{s}{\gt}{M}$ is the
        pair $(\gtlabel{p}{q}{m}\cdot w_1,M_r)$,
        where $\residat{s_1}{\gt}{M_1}=(w_1,M_r)$;
        \item otherwise, $\residat{s}{\gt}{M}=(\varepsilon,M)$
    \end{enumerate}
    The residuation $\resid{\gt}{M}$ of $M$ with respect to $\gt$ is
    $\residat{s_0}{\gt}{M}$, where $s_0$ is the initial state of $\gt$.
\end{defi}

Note that in condition 1 of Definition~\ref{def:residuation}, 
there is at most one tuple $(p,q,m,s_1,M_1)$ satisfying the condition, due to the
sender-driven choice, which ensures that $\residat{s}{\gt}{M}$ is uniquely defined.

\begin{exa}\label{example:residuation}
    Consider $\gt$  in Fig.~\ref{fig:example-of-sender-driven-gt-complementation}, and 
    $M_3=\mscof{\gtlabel{r}{r'}{b}\cdot\gtlabel{p}{q}{a_1}\cdot\gtlabel{p}{q}{a_3}}$ as in Example~\ref{ex:example-of-sender-driven-gt-complementation}.
    Then $\resid{\gt}{M}=(\gtlabel{p}{q}{a_1},M_r)$ where $M_r=\mscof{\gtlabel{p}{q}{a_3}\cdot\gtlabel{r}{r'}{b}}$.
\end{exa}
    

When $\resid{\gt}{M}=(w,M_r)$, we call $M_r$ the \emph{residual} of $M$ with respect to $\gt$, and $w$ its \emph{co-residual}. As we will later show, a sequence of arrows $w$
such that $\mscof{w}\not\in\existentialmsclanguageof{\gt}$ is in $\languageofnfa{\comp{\gt}}$ if and only if the co-residual of $\mscof{w}$ is a prefix of $w$. 

\begin{lem}\label{lem:residuation-and-acceptation}
    Assume $\resid{\gt}{M}=(w,M_r)$. Then
    $M\in\existentialmsclanguageof{\gt}$ if and only if
    $M_r$ is the empty MSC and $w\in\languageofnfa{\gt}$.
    %Moreover, when this holds, $w$ is the unique linearization of
    %$M$ in $\languageofnfa{\gt}$
\end{lem}

\begin{proof}
    For a state $s$ of $\gt$, let $\existentialmsclanguageof{\gt,s}$
    (resp. $\languageofnfa{\gt,s}$) denote the MSC language (resp. the language of arrows)
    accepted by $\gt$ with $s$ as initial state.
    Assume $\residat{s}{\gt}{M}=(w,M_r)$.
    By induction on the number of events of $M$, we show that for all state $s$ of $\gt$,
    $M\in\existentialmsclanguageof{\gt,s}$ if and only if
    $M_r$ is the empty MSC and $w\in\languageofnfa{\gt,s}$.

    \begin{itemize}
        \item Assume there are $p,q,m,s_1,M_1,w_1,M_r$ such that $M=\mscof{\gtlabel{p}{q}{m}}\cdot M_1$,
        and $(s,\gtlabel{p}{q}{m},s_1)$ is a transition of $\gt$,
        $\residat{s}{\gt}{M}=(\gtlabel{p}{q}{m}\cdot w_1,M_r)$,
        and $\residat{s_1}{\gt}{M_1}=(w_1,M_r)$. 
        By definition of $\existentialmsclanguageof{\gt,.}$, 
        if $M_1\in \existentialmsclanguageof{\gt,s_1}$, then $M\in\existentialmsclanguageof{\gt,s}$.
        By sender-driven choice hypothesis, conversely, if $M\in\existentialmsclanguageof{\gt,s}$,
        then $M_1\in \existentialmsclanguageof{\gt,s_1}$.
        By induction hypothesis
        $M_r$ is the empty MSC and $w_1\in\languageofnfa{\gt,s_1}$ if and only 
        $M_1\in \existentialmsclanguageof{\gt,s_1}$. As just observed, the later is equivalent
        to $M\in\existentialmsclanguageof{\gt, s}$; finaly, the former is equivalent
        to the fact that $M_r$ is the empty MSC and $w\in\languageofnfa{\gt,s}$ (because
        $\gt$ is deterministic), which ends the proof.

        \item Assume now that Condition 1 of Definition~\ref{def:residuation}
        does not hold, and $\residat{s}{\gt}{M}=(\epsilon, M)$. If $M$ is the empty
        MSC and $\varepsilon\in\languageofnfa{\gt,s}$, then 
        $M\in\existentialmsclanguageof{\gt,s}$. Conversely, if $M\in\existentialmsclanguageof{\gt,s}$
        and $M$ is not empty
        then Condition 1 of Definition~\ref{def:residuation} should hold, and the contradiction.
        Finaly, if $M\in\existentialmsclanguageof{\gt,s}$, $M$ is empty, but
        $\varepsilon\not\in\languageofnfa{\gt,s}$, we also get a contradiction.

    \end{itemize}
\end{proof}


\begin{lem}\label{thm:sender-driven-choice-complementation}
    Assume $\gt$ is a global type with sender-driven choices,
    and let $\renun{\gt}$ denote the global type defined as in Def~\ref{def:complement-of-a-sender-driven-gt}.
    Then $\renun{\gt}$ is a complement of $\gt$.
\end{lem}
\begin{proof}
    Let $\gt$ be a global type with sender-driven choice, and $\comp{\gt}$ its complement
    as defined in Definition~\ref{def:complement-of-a-sender-driven-gt}.
    Let $w\in\Arrows^*$ be fixed. Let $M,w_1,M_r,s,s_1,w_2$ be such that
    $M=\mscof{w}$, $\resid{\gt}{M}=(w_1,M_r)$, $\stateof{\comp{\gt}}{w}=s$, 
    $\stateof{\comp{\gt}}{w_1}=s_1$, and $w_2$ is the longest prefix of $w$ such that
    $\stateof{\gt}{w_2}$ is defined. The following properties are show by induction on the length of $w$.
    \begin{enumerate}
        \item If $w_1\neq w_2$, then $s=s_{\mathsf{rej}}$;
        \item if $w_1=w_2$ and $M_r$ is the empty MSC, then $s=s_1=\stateof{\gt}{w}$ is a state of $\gt$;
        \item if $w_1=w_2$, $M_r$ is not empty, 
        and $\senderof{\gt}{s_1}$ is undefined, then $s=s_{\mathsf{acc}}$;
        \item if $w_1=w_2$, $M_r$ is not the empty MSC, and $\senderof{\gt}{s_1}$ 
        is undefined, 
        then $s=s_{\mathsf{acc}}$;
        \item if $w_1=w_2$, $M_r$ is not the empty MSC, $\senderof{\gt}{s_1}=p$,
        and $M_r$ contains no $p$ events, then $s=\comp{s_1}$;
        \item if $w_1=w_2$, $M_r$ is not the empty MSC, $\senderof{\gt}{s_1}=p$,
        and the first $p$ event of $M_r$ is $\recv{q}{p}{m}$, then 
        $s=s_{\mathsf{acc}}$;
        \item if $w_1=w_2$, $M_r$ is not the empty MSC, $\senderof{\gt}{s_1}=p$,
        the first $p$ event of $M_r$ is $\send{p}{q}{m}$, and $\gtlabel{p}{q}{m}$
        does not label an outgoing transition of $s_1$ in $\gt$, then 
        $s=s_{\mathsf{acc}}$.
        \item if $w_1=w_2$, $M_r$ is not the empty MSC, $\senderof{\gt}{s_1}=p$,
        the first $p$ event of $M_r$ is $\send{p}{q}{m}$, $\gtlabel{p}{q}{m}$
        labels an outgoing transition of $s_1$ in $\gt$, and $\recv{p}{q}{m}$ is not 
        the first event of $q$, then 
        $s=s_{\mathsf{acc}}$.
    \end{enumerate}
    From the definition of accepting states of $\comp{\gt}$ and Lemma~\ref{lem:residuation-and-acceptation},
    it follows that 
    $$
        w\mbox{ is accepted by }\comp{\gt}\quad\mbox{if and only if}\quad 
        w_1=w_2 \mbox{ and } M\not\in\existentialmsclanguageof{\gt}.
    $$ 
    In particular, if 
    $M\in\existentialmsclanguageof{\comp{\gt}}$, then $M\not\in\existentialmsclanguageof{\gt}$.
    Conversely, let $M\not\in\existentialmsclanguageof{\gt}$ be fixed.
    There is a linearization of $M$ of the form $w=w_1\cdot w_r$ such that 
    $\resid{\gt}{M}=(w_1,\mscof{w_r})$. From the above properties,
    $\stateof{\comp{\gt}}{w}$ is accepting in $\comp{\gt}$, therefore $M\in\existentialmsclanguageof{\comp{\gt}}$,
    which ends the proof.
\end{proof}


